Quantitative Understanding of VAE as a Non-linearly Scaled Isometric Embedding

Variational autoencoder (VAE) estimates the posterior parameters (mean and variance) of latent variables corresponding to each input data. While it is used for many tasks, the transparency of the model is still an underlying issue. This paper provides a quantitative understanding of VAE property through the differential geometric and information-theoretic interpretations of VAE. According to the Rate-distortion theory, the optimal transform coding is achieved by using an orthonormal transform with PCA basis where the transform space is isometric to the input. Considering the analogy of transform coding to VAE, we clarify theoretically and experimentally that VAE can be mapped to an implicit isometric embedding with a scale factor derived from the posterior parameter. As a result, we can estimate the data probabilities in the input space from the prior, loss metrics, and corresponding posterior parameters, and further, the quantitative importance of each latent variable can be evaluated like the eigenvalue of PCA.

==> intro.tex <==
\section{Introduction}
Variational autoencoder (VAE) \citep{VAE} is one of the most successful generative models, estimating  posterior parameters of latent variables for each input data.
%Variational autoencoder (VAE) \citep{VAE} is one of the most successful generative models, estimating the posterior parameters (mean and variance) of latent variables corresponding to each input data.
%
In VAE, the latent representation is obtained by maximizing \mblu an evidence \mblk lower bound \mblu (ELBO). \mblk
%In VAE, the latent representation is obtained by maximizing \mblu an evidence \mblk lower bound of log-likelihood (ELBO). 
%
%A number of studies \citep{betaVAE, FactorVAE, HSIC-VAE, InfoGAN, TCVAE,   EchoNoise, INDUCTIVE_BIAS, VAEPCA} have  tried to reveal the property of latent variables.
%A number of studies \citep{betaVAE, FactorVAE, HSIC-VAE, TCVAE,   INDUCTIVE_BIAS, BELBO, VAEPCA} have  tried to reveal the property of latent variables.
%
%
\if0
A number of studies \citep{betaVAE, FactorVAE, HSIC-VAE, TCVAE,   INDUCTIVE_BIAS,  VAEPCA} have  tried to reveal the property of latent variables.
%A number of studies \citep{betaVAE, FactorVAE, HSIC-VAE, InfoGAN, TCVAE,   EchoNoise} have been tried to reveal the property of latent variable.
%The methods to acquire disentangled latent variables are also studied \citep{betaVAE, FactorVAE, HSIC-VAE, TCVAE, InfoGAN,  EchoNoise}. 
%
%Regarding the theoretical analysis, \citet{VAEPCA} prove that the Jacobi matrix of VAE is  orthogonal like principal component analysis (PCA).
%Regarding the theoretical analysis, \citet{VAEPCA} prove that the Jacobi matrix of VAE is  orthogonal.
%In the theoretical analysis, \citet{VAEPCA} prove that the Jacobi matrix of VAE is  orthogonal.
%\citet{VAEPCA} \mred \mblu proved theoretically that  the Jacobian \mblk  matrix of VAE is  orthogonal. 
%\citet{VAEPCA} prove theoretically that the Jacobi matrix of VAE is  orthogonal.
%
%
%\citet{INDUCTIVE_BIAS} \mred also \mblu proved  that unsupervised  \mblk representation learning essentially requires inductive biases on both models and data.  
%
%\citet{INDUCTIVE_BIAS} also prove that  unsupervised representation learning essentially requires inductive biases on both models and data.  
%
%To maximize ELBO, \citet{BELBO} analyzed the rate-distortion (RD) trade-off. 
%
%To maximize ELBO, \citet{BELBO} analysed the rate-distortion (RD) trade-off. 
%
%Here, Rate-distortion  theory \citep{RDTheory},  which is successfully applied to image compression, formulates that the RD trade-off optimum is achieved by using a PCA-like orthonormal transform.
%
%Here, \mblu RD \mblk theory \citep{RDTheory}, successfully applied to image compression, formulates that using a PCA-like orthonormal transform with uniform coding noise optimizes the RD trade-off.
%and is successfully applied to the transform coding for image/audio lossy compression. 
%
%Here, Rate-distortion  theory \citep{RDTheory} clearly formulates the optimal condition of the RD trade-off and is successfully applied to the transform coding for image/audio lossy compression. 
%
%\mblu Although \mblk the RD trade-off seems strongly related to RD theory, its relation was not discussed well.
%Although the RD trade-off seems strongly related to RD theory, they did not consider RD theory.
%Since they did not consider RD theory, the quantitative behaviour of VAE latent space is not clarified well.
%To maximize ELBO, \citet{BELBO} analysed the rate-distortion (RD) trade-off. 
%However, the quantitative behavior of the latent space at the optimum RD trade-off condition is still not clarified well.
%However, the quantitative behavior of the latent space  is still not clarified well.
%Since they did not consider RD theory, the quantitative behaviour of VAE latent space is not clarified well.
%While the RD trade-off in VAE seems strongly related to RD theory in the transform coding, it has been overlooked.
%previous  works did not consider the optimal condition formulated by RD theory. 
%
 \citet{BELBO}  also suggests that ELBO in VAE is broken and unstable. 
 However, quantitative behavior of VAE is still not well clarified.
For example,  there has not been a theoretical formulation of the reconstruction loss and KL divergence in ELBO after optimization.
More specifically,  although the conditional distribution $p_\theta(\bm x|\bm z)$ in the reconstruction loss of ELBO is predetermined such as the Gaussian or Bernoulli distributions, it has not been discussed well whether the true conditional distribution after optimization matches the predetermined distribution. 
%
\fi
%
%Furthermore, some works analysed the rate-distortion (RD) trade-off in ELBO.
%Here, Rate-distortion  theory \citep{RDTheory},  which is successfully applied to image compression, formulates that the RD trade-off optimum is achieved by a PCA-like orthonormal transform with constant posterior variance. However, their analysis seems inconsistent with RD theory.
%
Several theoretical studies have attempted to exactly characterize what is estimated by VAE.
Indeed, there are several unsolved questions, e.g., what is the meaning of the latent variable VAE obtained, what $\beta$ represents in $\beta$-VAE \citep{betaVAE}, whether ELBO converges to an appropriate value, and so on.
However, all of the existing researches failed to give answers to these important questions.
\citet{BELBO} \mblu introduced \mblk the \mblu RD \mblk trade-off based on the information-theoretic framework to analyse  $\beta$-VAE.
%
%However, the relation with \mblu the \mblk RD theory is not well discussed, and the quantitative properties of VAE are still unclear.
However, they did not clarify what VAE captures after optimization.
%
\citet{HiddenTalentVAE} showed VAE restricted as a linear transform can be considered as a robust PCA.
However, their model has a limitation for the analysis on each latent variable basis because of the linearity assumption. 
%
\citet{VAEPCA} \mblu showed \mblk the \mblu Jacobian \mblk matrix of VAE is orthogonal, which seems to make latent variables disentangled implicitly.
%
%\citet{VAEPCA} show that the Jacobi matrix of VAE is orthogonal like PCA, which makes latent variables disentangled implicitly.
%
However, they do not uncover the quantitative properties because they simplify KL divergence as a constant.
%
\citet{INDUCTIVE_BIAS} also showed \mblk the unsupervised learning of disentangled representations fundamentally requires inductive biases on both the metric and \mblu data\mblk. 
However, they do not uncover what kind of disentangled representations is obtained under the given inductive biases.
In non-VAE autoencoder studies, \citet{RaDOGAGA} propose an isometric autoencoder.
Their work seems to be related to VAE, however, it is not well clarified.

%in their analysis. 
%However, they do not uncover the orthonormality and quantitative properties since they assume a constant KL-divergence for easy analysis. 
%
%\citet{Diagnosing} also discussed the theoretical behavior of $\beta$ VAE for $r$ dimensional manifold when ideally trained, showing that the expected distortion and rate for $\beta \rightarrow 0$. 
%\citet{Diagnosing} also showed that the expected rate of VAE for the $r$-dimensional manifold is close to $-(r/2) \log \gamma + O(1)$ at $\gamma \rightarrow 0$ when $p_\theta(\hat {\bm x}| {\bm x}) = \mathcal{N}(\hat {\bm x}; {\bm x},\gamma I_m)$ holds.

In this paper, we resolve these essential problems by utilizing the view point of \emph{isometric embedding} \citep{NashThm2}.

1. First of all, we show that VAE obtains an implicit isometric embedding of the support of the input distribution as its latent space.
That is, the input variable is embedded through the encoder in a low dimensional latent space in which the distance in the given metric between two points in the input space is preserved.
%by scaling factor derived from the posterior parameter.  
Surprisingly, this characterization resolves most unsolved problems of VAE such as what we have enumerated above.
This implicit isometric embedding is derived as a non-linear scaling of VAE embedding.

2. More concretely, we will show the following issues via the isometric embedding characterization theoretically:
\\
(a) Rate-distortion optimal: VAE is the optimal encoding in the rate distortion sense such that the entropy of the implicit isometric embedding becomes minimum.
%since the entropy and the distortion are preserved in the isometric space. By analysing thawe show that VAE is the rate-distortion optimal $I(X, \hat X) = d(x, \hat {\bm x})$. 
\\
(b) Role of $\beta$ in $\beta$-VAE: $\beta$ controls each dimensional posterior variance of isometric embedding as a constant $\beta/2$.
\\
(c) Disentanglement: If the manifold has a separate latent variable in the given metric by nature, the implicit isometric embedding captures such disentangled feature as a result of minimizing the entropy.
\\
(d) Estimation of input distribution: the input distribution can be quantitatively estimated from that of the implicit isometric embedding because of the isometricity.

3. Finally, we justify our theoretical findings through several numerical experiments. 
We observe the estimated distribution is proportional to the input distribution in the toy dataset. 
By utilizing this property, the performance of the anomaly detection for real data is comparable to state-of-the-art studies.
We also observe that the variance of each dimensional component in the isometric embedding shows the importance of each disentangled property like PCA.
\if0
%\mblu RD \mblk theory \citep{RDTheory}, which is successfully applied to image compression, formulates that a PCA-like orthonormal transform with uniform coding noise optimizes the RD trade-off.
%Here, the transformed space is isometric  \citep{NashThm} where the distance and probability are the same as input space.
Rate-distortion (RD) theory \citep{RDTheory},  which is an important part of Shannon information theory and successfully applied to image compression, quantitatively formulates the RD trade-off optimum in lossy compression.
To realize a quantitative data analysis, Rate-distortion (RD) theory based autoencoder, RaDOGAGA  \citep{RaDOGAGA}, has been proposed  with isometric embedding \citep{NashThm}
where the distance between arbitrary two points of input space in a given metrics is always the same as L2 distance in the isometric embedding space.
%
%In this paper, we provide a clear understanding of VAE through non-linear mapping to RaDOGAGA. 
%In this paper, we provide a clear understanding of VAE by mapping VAE latent space to an implicit isometric space such as RaDOGAGA through non-linear scaling  on a variable-by-variable basis and analysing the quantitative property.
%
%In this paper, we provide a clear understanding of VAE by interpreting ELBO maximization as \mblu the RD \mblk optimization of transform coding based on RD theory. 
%
%By introducing an implicit isometric embedding,
%By introducing an implicit PCA-like orthonormal transform in VAE,
%
%We reveal the following traits theoretically and experimentally.
%We  thoroughly clarify VAE properties  theoretically and experimentally as follows.
%
%In this paper, by mapping VAE latent space to an implicit isometric space like RaDOGAGA on variable-by-variable basis and analysing VAE quantitatively as a well-examined lossy compression,
%

In this paper, by mapping VAE latent space to an implicit isometric space like RaDOGAGA on variable-by-variable basis and analysing VAE quantitatively,
we  thoroughly clarify the quantitative properties of VAE  theoretically and experimentally as follows.

%1) Implicit orthonormal transform is derived, such that the entropy of data representation becomes minimum  in the loss metric defined space.  A scaling factor between  VAE  and the implicit orthonormal transform is formulated by the  posterior parameters for the corresponding input data.
1)
An implicit isometric embedding is introduced in the loss metric defined space such that the entropy of data representation becomes minimum. 
A scaling factor between the VAE latent space and implicit isometric space is formulated by the posterior for each input.
%We also show that the posterior variance of each dimensional component in the implicit isometric embedding space is a constant $\beta/2$.
%We also show that the posterior variance of each dimensional component in the implicit isometric embedding space is a constant.
In the case of $\beta$-VAE, the posterior variance of each dimensional component in the implicit isometric embedding space is a constant $\beta/2$, which is analogous to the rate-distortion optimal of transform coding in RD theory.
%As a result, the reconstruction loss and KL divergence in ELBO can be quantitatively formulated.
As a result, the reconstruction loss and KL divergence in ELBO can be deterministically quantified, implying ELBO is not broken.
%This also corrects the theoretical analysis of some prior works \citep{ BELBO}.
%the optimized $\beta$-VAE adds the noise $\beta/2$ equally to each dimension of isometric embedding, consistent with RD  theory.
%We also show  the optimized $\beta$-VAE adds the noise $\beta/2$ equally to each dimension of isometric embedding, consistent with RD  theory.
%It is also shown that ELBO is maximized in the loss metric defined space instead of the input space.
\\
%1) Implicit orthonormal transform is derived as a PCA/KLT of  data in the loss metric defined space.
%2) A scaling factor between the VAE encoder/decoder and the implicit orthonormal transform can be formulated by the variances of posterior distribution parameters for the corresponding input data. \\
2)
From these properties, VAE can provide a practical quantitative analysis of input data.
%
First, the data probabilities in the input space can be estimated from the prior, loss metric, and  posterior parameters.
%
In addition, 
%if the data manifold has a disentangled feature by nature in the given metric, 
the quantitative importance of each latent variable, analogous to the eigenvalue of PCA, can be evaluated from the posterior variance.
%2) The quantitative importance of each latent variable, analogous to the eigenvalue of PCA, can be evaluated from the statistical value of distribution parameters.\\
%In addition, the data probabilities in the input space can be estimated from the prior, loss metrics, and  posterior parameters.
%2) The quantitative importance of each latent variable, analogous to the eigenvalue of PCA, can be evaluated from the posterior variance.\\
%3) The data probabilities in the input space can be estimated from the prior, loss metrics, and  posterior parameters.
%We believe that these quantitative features will spur a new solution for practical \mred applications. \mblk 
%tasks. 
%
\\
3) 
From 1), We prove that the predetermined conditional distribution for the reconstruction loss in the original VAE matches the true conditional distribution after optimization. By contrast, both distributions in $\beta$-VAE with $\beta \neq 1$ are not equal.  Instead, what $\beta$-VAE really does is only to scale the variance of the pre-determined conditional distribution in the original VAE by a factor of $\beta$.

%
\fi
%This work will lead the information theoretic generative models in the right direction.

\if0
1) WeAn implicit orthonormal transform is introduced. a scaling factor between the VAE encoder/decoder and the implicit orthonormal transform can be formulated by the distribution parameters
Probabilities of samples can be estimated by the product of the prior's probability value at $\mu$ and the value of $\sigma$.\\
2) The impact of each latent variable on the real space, which is analogous to eigenvalue of PCA, can be estimated by the average of $\sigma^{-1}$ in the corresponding channel.\\
3) Rate-distortion optimized latent space is defined by both data feature and metrics of reconstruction loss.  These two will be corresponding to the inductive biases on both the models and the data as shown in \citet{INDUCTIVE_BIAS}.
\fi
%
\if0
多次元の複雑なデータの本質的な特長や表現を獲得することは、機械学習の基本となる。
その中でも、生成モデルアプローチは潜在表現と確率分布を獲得し、サンプリングは教師無し／弱教師学習等への適用を目的とされている。そして、特にDisentangleなどのメタPriorなどの学習も目的とされている。
この中でVAEは、教師無しの生成モデルや表現学習として、もっとも成功したものである。そして、Disentangleを目的として、β-VAR、FactorVAEなどが提案されてきた。そしてその最適化については、AlemiなどがRate-Distortion理論で説明を試みてきた。また、潜在変数の理解に関する研究も進み、Rolinekらが、Jacobianが直交し、PCAの特長を有するということをしめした。
  しかし、VAEの潜在空間の定量的な解釈の研究は進んでいるとはいえない。たとえば、潜在空間で現れる確率分布と実空間との確率の関係や、reparametizatin trickで現れるσの意味などの理論的な解釈は未解明のままである。
  
  一方、画像・音響などの情報圧縮では、RD理論が長年研究され、この理論に基いた変換符号化が成功を収めていた。変換符号化では、KLTやDCTといった直交変換で入力信号を変換して無相関化したのちに、各チャネルの誤差が等しくなるように量子化し、各シンボルの生起確率に応じたエントロピー符号化により情報圧縮するものである。
  本論文では、理論的に確立した変換符号化の理論をスタートポイントとしてVAEを理解することにより、VAEの潜在変数や確率分布の解釈を与えることを目的とする。具体的には、オリジナルのRD最適化理論で想定されている直交変換符号化と量子化・符号割り当てからなる符号化モデルとそのRD最適化条件を想定する。そして、VAEと関連付け、VAEのDKLが量子化・符号割り当てプロセスと解釈することで、σや潜在空間と実空間との定量的な関係を明らかにする。そして、Toyデータおよび実データでRD理論とVAEとの関連付けから想定されると定量的に一致することを示すことで仮説を立証し、VAEが変換符号化のRD最適化条件でもとめた潜在変数の各スケールを非線形変換したものとして解釈可能である証拠として示す。
\fi



==> math_commands3.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\argmin}{\mathop{\rm arg~min}\limits}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> rebuttal.tex <==
%We thank all the reviewers for their careful reviews and valuable feed-backs. 
%Since we take reviewers' comments seriously and promise to revise carefully as detailed below.
%Please note that "(R$n$)" denotes our response to the reviewer \#$n$.
We thank all the reviewers for their careful reviews and valuable feedback. In the following we address their concerns. We will revise the manuscript reflecting these points. 
Please note that "(R$n$)" denotes our response to the reviewer \#$n$. 
\\
%, we would appreciate it if reviewers could consider the possibility of the improvements.\\
%R~~の書き方は一般的なので省略可
%最初にレビュワーのコメントに沿って、と書いて、最後にour instituteにした方が良い
%
%Response to Reviewer 1:\\
%
%
%\textbf{Response to Reviewer 4:}\\
%
%\begin{eqnarray}
\if0
\textbf{Organization of the paper (R1):}
%We would appreciate read again the 
%First of all, 
We believe the reason you felt the difficulty would be solved once you understand our motivation.
%We would like to clarify our motivation. 
Although (beta-)VAE has been widely used in many area, the quantitative relation between the latent variable and the input data has been not been theoretical analyzed. 
Therefore, to improve the performance in practical tasks such as the anomaly detection or data interpolation, prior work rely on empirical method. Note that, even in GMVAE or DAGMM does not guarantee how the latent variable correctly capture the character of the data. 
RaDOGAGA (Kato et al., 2020), insisted that the isometric embedding is key point to solve this matter. 
Although they mentioned VAE lacks this property, our theoretical investigation dug out that VAE can be mapped into isometric embedding. 
The paper is organized so that prove this finding. 
%Our experimental result showed 

\fi
%In the related work
\if 0
\textbf{Organization of paper:}
%※多分、この項目ひっくり返らない気がします
Reviewers concern the organization paper. 
%One expected reason is we put to much equation or proof in the main paper. We can move some proof completely in the appendix. 
%One expected reason is we missed to clarify the motivation. 
In the extra space for the camera ready, we can put the motivation or intuitive explanation. 
For instance, the reason we mentioned the analogy to the Wiener filter theory is that in the optimal condition, VAE behaves Wiener filter that further supports the validity of interpreting VAE in the context of transform coding theory. 
\fi
%
\textbf{Organization of paper(All):}
%Given a reviewer's response, we asked some researchers in our institution to give us advice. 
%Given a reviewer's response, we asked some researchers for advices. 
%Based on that, we can put intuitive explanation after proof or the lemma. 
%Particularly, we will add following explanation:
\if0
%Based on advice from some researchers in our institute, 
Based on the R1's comment, we will put an intuitive explanation after the proofs
%Based on that, we will put an intuitive explanation after the proof and lemma,  
particularly as follows:
(i) After the theory 1: This theory indicates that the mapping of the VAE has a property which is similar to isometric embedding. 
(ii) After the theory 3: $\beta$ in beta-VAE eventually determines the degree of distortion in each axis. 
\fi
%Based on advice from some researchers in our institute, we will put an intuitive explanation after the proofs. 
Based on the R1's comment we will put an intuitive explanation after the proofs. 
%For example, after the proof of Lemma 4, we add a description that ``This Lemma shows not only the orthogonality but the norm of $\bm x _{\mu_j}$. 
For example, after the proof of Lemma 4, we will add ``This Lemma shows not only the orthogonality but the norm of $\bm x _{\mu_j}$. 
Thus the implicit isometric embedding is derived by dividing $\bm x _{\mu_j}$ by the norm". 
In addition, we will add the detailed relationship and differences with RaDOGAGA according to the R1's comment. 
%We also promise to correct typos including R5's comments and describe the full name of an abbreviation  after careful check.
We also fix typos, correct the incorrect description pointed out in the R5's comments, and describe the full name of an abbreviation after careful check. %In addition, we have asked several researchers in our institute. 
%We will also fix typos and incorrect descriptions including the one pointed out by R5, and describe the full name of abbreviations as suggested by R6. In addition, we have asked several researchers in our institute advise on writing. 
\\
%For instance, after the proof of theory 1, we will explain that the mapping of the VAE has a property which is similar to isometric embedding. 
%For another instance, after the proof of theory3, we will add that the beta determines the capacity of the error in each axis.
%For instance, the reason we mentioned the analogy to the Wiener filter theory is that in the optimal condition, VAE behaves Wiener filter that further supports the validity of interpreting VAE in the context of transform coding theory. //
%\textbf{Arbitrary Prior rather than Gaussian (R1):} 
\textbf{Non-Gaussian prior (R1):} 
%When $D_\mathrm{KL}(\cdot)$ is replaced by the second equation of Eq.~9, our theoretical analysis is valid for arbitrary priors. 
%Our theoretical analysis is valid for an arbitrary prior such that the approximation in the second line of Eq.9 is held. 
\if0
Our theoretical analysis is valid for an arbitrary prior since the approximation in the second line of Eq.9 is always held. 
The posterior variance  $\sigma_j$ bridges between the distributions of data and prior, as in Eq.~17.
If the prior is set close to the data distribution, $\sigma_j$ becomes close to constant, which facilitates  training.
\fi
Our theoretical analysis is valid for an arbitrary prior since the approximation in the second line of Eq.9 is always held, since $D_\mathrm{KL}(\cdot) = \int q(\cdot) \log p(\cdot)  \mathrm{d}z  -\int q(\cdot) \log q(\cdot) \mathrm{d}z  \simeq \log p(\cdot) + \sum \log \sigma_j \sqrt{2 \pi e}$ will hold where $q(\cdot)$ act like a delta with small $\sigma_j$. 
We add this proof.
% 
The posterior variance  $\sigma_j$ bridges between the distributions of data and prior, as in Eq.~17.
If the prior is set close to the data distribution, $\sigma_j$ becomes close to constant, which facilitates  training.
\\
\textbf{Decomposed loss derivation (R7):}
%We add the next explanation. 
%Assume or Simplisityは必須 
%Consider the case ${{}^t \bm x} \bm G_x {\bm x}=||{\bm x}||_2^2$ for simplicity
Assume $||{\bm x}||_2^2= {{}^t \bm x} \bm G_x {\bm x}$ holds in the metric space of $\bm G_x$. 
%Assume the metric space of $\bm G_x$ where $||\vx||_2^2= \vx \bm G_x \vx$ holds. 
%Using $1_{st}$  order expansion of $\hat \vx$ with  $\delta {z_j } \sim \mathcal{N}(0,\sigma_j)$,  
Using Taylor expansion of $\hat {\bm x}$ with  $\delta {z_j } \sim \mathcal{N}(0,\sigma_j)$,  
$D({\bm x}, \hat {\bm x})= 
||\bm x - \hat {\bm x}||_2^2 =
||(\bm x - \breve {\bm x})+(\breve {\bm x} - \hat {\bm x})||_2^2 \simeq
||\bm x - \breve {\bm x}||_2^2 +||\breve {\bm x} - \hat {\bm x}||_2^2 + \sum 2 \delta {z_j }\ {}^t (\bm x - \breve {\bm x}) \bm G_x {\bm x}_{\mu_j}$
 holds.
% $D_\mathrm{KL}(q_\phi(\vz|x)||$
 %using $\delta {z_j } \sim \mathcal{N}(0,\sigma_j)$.  
Since the average of $\sum \cdot \ $ term over $\delta {z_j }$ is 0,
%$|\bm x - \hat \vx|_2^2 \simeq |\bm x - \breve \vx|_2^2 +|\breve \vx - \hat \vx|_2^2$ holds.\\
%$E_{\delta {z_j }}[D(\bm x,\hat \vx)] \simeq E_{\delta {z_j }}[D(\bm x,\breve \vx)] +E_{\delta {z_j }}[D(\breve \vx, \hat \vx)]$ holds.\\
$E_{\delta {z_j }}[D(\bm x,\hat {\bm x})] \simeq E_{\delta {z_j }}[D(\bm x,\breve {\bm x}) + D(\breve {\bm x}, \hat {\bm x})]$ holds.
We add this proof.
\\
%
%\nonumber
%\end{eqnarray}
%
\textbf{Understanding of dimension with $D_{\mathrm{KL}j}(\cdot)=0$ (R7):}
%reviewerは図4の読み方を誤解している可能性がある
%$D_\mathrm{KL}(\cdot)=0$ならVariance=0であることを伝えて、横軸が次元のindex(降順であること)を確認した方が良いかも。
%Number⇒index
%The latent dimensional component with $D_\mathrm{KL}(\cdot)=0$, i.e., $\sigma_j=1$ and $\mu_j=0$, can be considered that the variance of its implicit isometric latent variable $\mathrm{Var}(y_j)$ is less than the implicit posterior variance $\beta/2$.
% In beta-VAE, some latent variables could be unneccesary. have information. In such dimension, $D_\mathrm{KL}(\cdot)=0$. 
%In beta-VAE, some latent variables could be unnecessary. $D_\mathrm{KL}(\cdot)=0$ is the condition to be such dimension. In these dimensions, the variance of its implicit isometric latent variable $\mathrm{Var}(y_j)$ is less than $\beta/2$ (the implicit posterior variance in theory). 
%Some variables will lose information when $D_\mathrm{KL}(\cdot)=0$. In that case, the norm. 
%In the dimensions where $D_\mathrm{KL}(\cdot)=0$, variables does not convey information. Thus, the norm of $\vx_{yj}$ is also 0, not 1. In such dimensions, the latent variable $\mathrm{Var}(y_j)$ is less than the implicit posterior variance which is $\beta/2$ in theory. 
%The latent dimensional component with $D_\mathrm{KL}(\cdot)=0$  can be considered that the variance of its implicit isometric latent variable $\mathrm{Var}(y_j)$ is less than the implicit posterior variance which is $\beta/2$ in theory.
%The latent dimension with $D_\mathrm{KL}(\cdot)=0$  can be considered that the variance of its implicit isometric latent variable $\mathrm{Var}(y_j)$ is less than the implicit posterior variance which is $\beta/2$ in theory.
%
%If ``variance" in R7 comment is estimated variance $Var(y_{j})$, $D_\mathrm{KL}(\cdot)=0$ when $Var(y_{j})$ is small. 
%Note that x-axis in Fig.~4 is index of dimension sorted by ``descending" order of $Var(y_{j})$. 
%If ``variance" is ${\sigma_{z_j}}^2$, the following clarification is given. 
%
%%%%%%%%%
%
\if0
First, let us clarify that ``Variance" in Figs. 4 and 5 is an estimated variance $\mathrm{Var}(y_{j}) = E[{\sigma_{j(\bm x)}}^{-2}]$ for the implicit isometric variable in Eq.~20.
%In the latent dimension with $D_\mathrm{KL}(\cdot)=0$, the variance of its implicit isometric latent variable $\mathrm{Var}(y_j)$ will be less than the implicit posterior variance which is $\beta/2$ in theory.
In the latent dimension with $D_\mathrm{KL}(\cdot)=0$,  $\mathrm{Var}(y_j)$ will be less than the implicit isometric posterior variance which is $\beta/2$ in theory.
%This can be explained from Rate-distortion theory for transform coding in Appendix B.6.
This can be explained from Rate-distortion (RD) theory in Appendix B.6.
In Eq.~88 of RD theory, if the latent variable's variance  ${\sigma_{z_j}}^2$ is less than the posterior variance $d$,  a rate $R_{opt}$ is $0$.
%Since $D_{\mathrm{KL}j}(\cdot)$ can be approximated as a rate as in Appendix A.2, $\mathrm{Var}(y_j)$ will be less than $\beta/2$ in a dimension with $D_{\mathrm{KL}j}(\cdot)=0$.
Since $D_{\mathrm{KL}j}(\cdot)$ can be approximated as a rate as in Appendix A.2, 
%$D_{\mathrm{KL}j}(\cdot)=0$ will be observed in a dimension where $\mathrm{Var}(y_j)$ is less than the posterior variance.
$D_{\mathrm{KL}j}(\cdot)=0$ will be observed if $\mathrm{Var}(y_j)$ is less than the implicit isometric posterior variance.
Thus, if $D_{\mathrm{KL}j}(\cdot)=0$, the norm in the first term of Eq.~12 will be 0 since the norm term does not have to be balanced with $D_{\mathrm{KL}j}(\cdot)$ anymore.
\\
%Then, if $\beta$ becomes smaller, the number of meaningful dimensions increases where $D_\mathrm{KL}(\cdot)>0$, i.e., $\mathrm{Var}(y_j) > \beta/2$ holds,  
%Then, if $\beta$ becomes smaller, the number of meaningful dimensions increases where $\mathrm{Var}(y_j)$ is larger than the posterior variance.  
Then, if the posterior variance becomes smaller, the number of meaningful dimensions with $D_\mathrm{KL}(\cdot)>0$ will increase.  
%\\
The  difference of meaningful dimensions  between  Figs.~4 and 5 is explained as follows:
the posterior variance in Fig.~5 is almost $\beta/2$; however, the posterior variance in Fig.~4 is  $1.83$ times larger than $\beta/2$.
Thus, the meaningful dimensions in Fig.~4 is less than those in Fig.~5.
Figure~25 also shows the CelebA results with smaller $\beta$, where all dimensions are meaningful. \\
\fi
%%%%%%%
%
\if0
・VAEでは、要らない次元が出た時、情報を持たない次元、つまりノルムが0になる次元が生じる。
%・Remark2はこの条件を述べている(Ｄ_kl(\dot) = 0)
・これはimplicitな空間では、Var < β/2と等価である。
・なので、Varが図4のものをさすとき、Varが小さい時にがこの条件が発生する。
・図4でノルムが0の次元は、画像の変化にも影響を及ぼさない
・逆に言うと、βが大きい(再構成を綺麗にしようとする)とこの条件は発生しにくい。
%・もっと直感的には、と条件は発生しにくい。
・図５ではdecomposed lossは綺麗な再構成を促すので、条件が発生しにくくなっている。
%%%%%%%%%%%%%%%%%%
・まずNormがゼロになる理由を説明する。
・EQ12で第一項はNorm、第二項はDKL。
%DKLとreconstracution error(norm)のバランスによって学習が行われる
%
・DKLがゼロになると、EQ12はバランスする必要がないので、Normはゼロになる。
%この場合、該当の次元は情報を持たない
・次にDKLがゼロになる条件は、固定値である等長空間のPosterior Varianceを
  閾値として、この閾値より潜在等長空間の変数の分散が小さい場合となる。
・これは、Appendix A.7とB.6で説明している。
・最後に、Fig4とFig5の違い。
・Fig5のDecomposed Lossを用いると、Posterior Varianceは理論通りのβ／２
  となっている。
・この場合、たまたまこのデータでは、すべての次元で等長変数の分散がβ／２より
  おおきいので、Normはすべてゼロでない。
・一方、Fig4の場合には、Posterior Varianceは理論値の1.83倍となる。
・閾値が大きくなったので、これより小さい次元がでてしまい、Fig４では
  Normがゼロになる次元がでてくる。
\fi
%
%%%%%%%
%
First, we explain why the norm becomes 0 when  $D_{\mathrm{KL}j}(\cdot)=0$.
%In Eq.~12, the first term for the norm scaled by $2/\beta$ and the second term for $D_{\mathrm{KL}j}(\cdot)$ are balanced.
The loss in Eq.~12 is a summation of the norm (multiplied by $\beta/2$) and  $\beta D_{\mathrm{KL}j}(\cdot)$, where both terms are balanced.
If $D_{\mathrm{KL}j}(\cdot)=0$, the norm also becomes zero because balancing is no more needed. 
Second, we explain the condition where $D_{\mathrm{KL}j}(\cdot)=0$.
Let $\mathrm{Var}(y_j)$ and ${\sigma_{y_j(x)}}^2$ be the variance and posterior variance of $j$-th implicit isometric component ${y_j}$, respectively.
Here, ${\sigma_{y_j(x)}}^2$ is $\beta/2$ in our theory.
Then the condition where $D_{\mathrm{KL}j}(\cdot)=0$ is derived as $\mathrm{Var}(y_j) \le {\sigma_{y_j(x)}}^2$, as shown in Appendix A.7 and Appendix B.6 (RD theory).
In RD theory, this is corresponding to the case where the signal magnitude is always less than quantizer and no information is needed to encode.
Finally, we explain the reason why the behaviors in Figs.~4 and 5 are different.
In Fig.~5 with the decomposed loss, ${\sigma_{y_j(x)}}^2$ is almost $\beta/2$ as theory expected.
In this case,  all of $\mathrm{Var}(y_j)$ happen to be greater than ${\sigma_{y_j(x)}}^2$.
In Fig.~4 with the conventional loss, however, ${\sigma_{y_j(x)}}^2$ is about 1.83 times greater than $\beta/2$.
Note that  $\mathrm{Var}(y_j)$ in  both Figs.~4 ad 5 cases will be almost the same because of the isometric embedding with minimum entropy.
Since ${\sigma_{y_j(x)}}^2$ becomes larger, the number of dimensions where  $\mathrm{Var}(y_j) \le {\sigma_{y_j(x)}}^2$ will increases. 
Accordingly, the dimensions where the norms are zero also increase.
Figure~25 also shows the CelebA results with smaller $\beta$, resulting smaller ${\sigma_{y_j(x)}}^2$. Here, all dimensions have nonzero norms since $\mathrm{Var}(y_j)  > {\sigma_{y_j(x)}}^2$ will hold. 
%
%
%%%%%%%
%
\if0
First, let us clarify that ``Variance" in Figs. 4 and 5 is an estimated variance $\mathrm{Var}(y_{j}) = E[{\sigma_{y_j(\bm x)}}^{-2}]$ for the implicit isometric variable in Eq.~20.
%In the latent dimension with $D_\mathrm{KL}(\cdot)=0$, the variance of its implicit isometric latent variable $\mathrm{Var}(y_j)$ will be less than the implicit posterior variance which is $\beta/2$ in theory.
In the latent dimension with $D_\mathrm{KL}(\cdot)=0$,  $\mathrm{Var}(y_j)$ will be less than ${\sigma_{j(\bm x)}}^2$, the posterior variance of implicit isometric variable which is $\beta/2$ in theory.
%This can be explained from Rate-distortion theory for transform coding in Appendix B.6.
This can be explained from Rate-distortion (RD) theory in Appendix B.6.
In Eq.~88 of RD theory, if the latent variable's variance  ${\sigma_{z_j}}^2$ is less than the posterior variance $d$,  a rate $R_{opt}$ is $0$.
%Since $D_{\mathrm{KL}j}(\cdot)$ can be approximated as a rate as in Appendix A.2, $\mathrm{Var}(y_j)$ will be less than $\beta/2$ in a dimension with $D_{\mathrm{KL}j}(\cdot)=0$.
Since $D_{\mathrm{KL}j}(\cdot)$ can be approximated as a rate as in Appendix A.2, 
%$D_{\mathrm{KL}j}(\cdot)=0$ will be observed in a dimension where $\mathrm{Var}(y_j)$ is less than the posterior variance.
$D_{\mathrm{KL}j}(\cdot)=0$ will be observed if $\mathrm{Var}(y_j)$ is less than the implicit isometric posterior variance.
Thus, if $D_{\mathrm{KL}j}(\cdot)=0$, the norm in the first term of Eq.~12 will be 0 since the norm term does not have to be balanced with $D_{\mathrm{KL}j}(\cdot)$ anymore.
\\
%Then, if $\beta$ becomes smaller, the number of meaningful dimensions increases where $D_\mathrm{KL}(\cdot)>0$, i.e., $\mathrm{Var}(y_j) > \beta/2$ holds,  
%Then, if $\beta$ becomes smaller, the number of meaningful dimensions increases where $\mathrm{Var}(y_j)$ is larger than the posterior variance.  
Then, if the posterior variance becomes smaller, the number of meaningful dimensions with $D_\mathrm{KL}(\cdot)>0$ will increase.  
%\\
The  difference of meaningful dimensions  between  Figs.~4 and 5 is explained as follows:
the posterior variance in Fig.~5 is almost $\beta/2$; however, the posterior variance in Fig.~4 is  $1.83$ times larger than $\beta/2$.
Thus, the meaningful dimensions in Fig.~4 is less than those in Fig.~5.
Figure~25 also shows the CelebA results with smaller $\beta$, where all dimensions are meaningful. \\
\fi
\\
%
%%%%%%%%%%
%
\textbf{Increase of latent dimension (R7):}
The next table and figure show the results using Table 1 condition except the latent dimension is increased to 5.
For $z_1$ to $z_3$, each value is close to Table 1.
%For $z_4$ and $z_5$, norm values are almost 0 and the variances are close to 1.
For $z_4$ and $z_5$, $({2}/{\beta}){\sigma_{j}}^{2} {D^{\prime}}_j$ are almost 0 and  the averages of $ {{\sigma_{{j}(\bm x)}}}^{-2} $ are close to 1.
In such dimensions,  $\mathrm{Var}(y_j) < \beta/2$ and $D_{\mathrm{KL}j}(\cdot)=0$ will hold as explained above.
The figure describes the plot for ${a_x}^{n/2}\exp(-L_{\bm x} / \beta)$ corresponding to Fig.~3 (d), also showing almost proportionality.
%
\begin{figure}[h]
    \begin{minipage}[b]{0.6\linewidth}
%	\caption{Property measurements of the  toy dataset \\  trained with the square error loss.}
	%\caption{Measurements of VAE properties \\for the toy dataset  trained with the square error loss.}
%	\label{TBL_TOY1}
	\begin{tabular}{r|lllll}
	 variable \hspace{2mm} & $z_1$	& $z_2$	& $z_3$ & $z_4$	& $z_5$ \\  \hline \hline
%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	$\frac{2}{\beta}{\sigma_{j}}^{2} D^{\prime}_j$ \hspace{1mm} Av.
%	$\frac{2}{\beta}{\sigma_{j(\bm x)}}^{2} D^{\prime}_j(\bm z)$ av.
%	${}^t{{\bm x}_{y_j}} \bm G_x {{\bm x}_{y_j}}$ av.
%		& 0.1451 & 0.5872 & 2.268 \\
		& 0.963 & 0.918 & 0.964 & 0.000 & 0.000 \\
 	SD 
% 		& 0.0425	& 0.3697	& 1.401 \\ \hline
 		& 0.053 	& 0.169 	& 0.103 & 0.000 & 0.000 \\ \hline
%%%%
%	\addlinespace[1mm]
%	$\frac{2}{\betaa]{\sigma_{(\bm x)j}}^{2} D^{\prime}_j(\bm z)$ \hspace{2mm} avg. 
%		& 0.1935	& 0.7829	& 3.023 \\
%		&4.99e-4	& 4.76e-4	& 4.99e-4 \\
%
%	 sd.	
%	 	& 5.660e-2	& 4.929e-2	& 1.868 \\
%	 	&2.24e-5	& 8.94e-5	& 3.88e-5 \\
%	\addlinespace[1mm]
%	$ \sqrt{\overline {{\sigma_{(\bm x)j}}^-2}}$ \hspace{15mm}	 &19.05	& 38.35	& 75.44 \\ 
	$ {\sigma_{j(\bm x)}}^{-2} $ \hspace{2mm}	 Av.
%		&3.33e+1	& 1.46e+2	& 5.89e+2 \\
		&3.34e1	& 1.46e2	& 5.88e2  & 1.00e0 & 1.00e0\\
    {\footnotesize (Ratio)}	Av.
    	& 1.0	& 4.39	& 17.69 & 0.03 & 0.03\\ \hline
	\end{tabular}
\end{minipage}
\if0
\begin{minipage}{0.38\textwidth}
\begin{center}
\makeatletter
\def\@captype{table}
\makeatother
\begin{tabular}{|l|c|r|}
\hline
a & b & c \\ \hline
d & e & f \\ \hline
g & h & i \\ 
\hline
\end{tabular}
\caption{sample}
\label{label 2}
\end{center}
\end{minipage}
\fi
%
\begin{minipage}{0.35\textwidth}
\begin{center}
\includegraphics[width=35mm]{figs/Bottom5.png}
%\subcaption{graphic 1}
\label{label 1}
\end{center}
\end{minipage}
\end{figure}
\\
\textbf{Approximation for large ${{\sigma_{{j}(\bm x)}}}$ (R1, R7):} 
Our approximation will break in a dimension where ${{\sigma_{{j}(\bm x)}}}$ is close to 1. 
%Our approximation breaks where $\sigma_j$ is close to 1. 
Note that VAE has an essential problem in such ${{\sigma_{{j}(\bm x)}}}$ range, since the prior and posterior are too close to capture exact information. 
%The next response could be a solution.
%the posterior variance act as a gauge t
\\
\textbf{Control of information (R1, R7):} 
${\beta/2}$ acts as a minimum scale of ruler to analyze latent space.
%If one wants to analyse specific features, the following procedure will 
%The following procedure find the dimension with no information. 
%The following procedure will adjust the information in the specific dimension
%The following procedure is reasonable to examine a particular dimension in more detail.
%The following procedure will adjust the information and solve the ill-manner behaviour in the dimensions  where $\sigma_j$ is close to 1 (but less than 1).
The following procedure will adjust the information  in the ill-mannered dimensions  where $\sigma_{j(x)}$ is close to 1, but less than 1.
(1) Train $\beta$-VAE with appropriate $\beta$. 
%(2) Identify the dimensions for detailed analysis, for example, by Eq.~20 or $D_{\mathrm{KL}j}(\cdot)$. 
(2) Identify the dimensions for detailed analysis by $D_{\mathrm{KL}j}(\cdot)$ or average $\sigma_{j(x)}$. 
(3) Replace $\beta D_\mathrm{KL}(\cdot)$ in Eq.~3 by $\sum \beta_j D_{\mathrm{KL}j}(\cdot)$ to control  a minimum scale ${\beta_j/2}$ in each dimension individually. 
$\beta_{j}$ is set to $\beta$ by default, but decrease $\beta_{j}$ from  $\beta$ in the dimensions for  detailed analysis.
(4) Conduct fine-tune.
Then only the target dimensions will be rescaled.
%Then the scale will be enlarged via $\beta_j$.
%These procedure will solve the ill-manner in a dimension where $\sigma_j$ is close to 1.
\\
\textbf{Distance in low density region (R6):}
%保証していないが、成り立つ可能性がある。実際、figc,dでは捉えている。
%In the low density area, distance learning may fail.
%Please note that Figs.~3 (c)(d) seem to capture a distance appropriately even in low density area since the proportionality is also  well shown there.
In the low density area, distance is not ensured, but may be learned. 
In Figs.~3 (c)(d), the model captures a distance appropriately even in low density area since the proportionality is also well shown there.
\\
%\if 1
\textbf{``Disentanglement" (R6):}
Previous disentangle metrics is based on intuitive attributes like ``shape", ``size", and so on. 
We define the ``disentangled" as independent to represent data like PCA, regardless of whether it is intuitive for the human or not.
%\\
\begin{wrapfigure}{r}[0pt]{60mm}
% \begin{center}
  \includegraphics[width=60mm]{figs/GaussTheorem.jpg}
%  \raisebox{-15.5zw}[0pt][15.5zw]{\includegraphics[clip,width=60mm]{figs/GaussTheorem.jpg}}
%  \raisebox{10mm}{\includegraphics[width=60mm]{figs/GaussTheorem.jpg}}
%\end{center}
\end{wrapfigure}
%%%%
%
\textbf{Larger $\beta$ captures global feature (R1):}
%We have the same question, and our intuition is as follows:
Our intuition is as follows:
Assume 2D manifold in 3D space, where isometric embedding is governed by Gauss curvature.
Please see the right figures. 
If large $\beta$, $\beta$-VAE will capture global features with lower entropy allowing large distortion.
If small $\beta$, however, $\beta$-VAE can capture only fragmented features allowing small distortion. 
We  assume similar behaviors in higher dimensional manifold.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\if 0

\textbf{Definition of ``Disentanglement" (R6):}
%3行番：かなり分かりにくいと思うので、出来れば4行にしたいです。
%In our work, ``disentagled'' is only determined given metric and data
The disentangle metric in previous works is based on the attributes pre-determined by human, such as ``shape", ``size", and so on, ignoring whether these attributes are truly independent to reconstruct data. 
We clarify the ``disentangled" as independent to represent data like PCA, regardless of it is intuitive for the human or not.

\textbf{Definition of ``Disentanglement" (R6):}
The disentangle metric in the factor VAE or beta-VAE is based on the attribute which is pre-determined by human, such as ``shape", ``size", and so on. 
Whether these attributes are truly independent to reconstruct data under the given distance function is unclear. 
On the other hand, in the PCA, each component is independent to represent data, regardless of whether it is intuitive for the human or not. We clarify ``disentangled" in our study is the latter one. 

%一応書きました。余白が残れば
\textbf{Why Anomaly detection is chosen (R6):}
In the anomaly detection task, the accurate estimation of probability density function (PDF) of data is the key issue, which can be encouraged by isometric embedding. 
The good performance in this task not only validates our theory but also the practical benefit that VAE can be mapped to isometric embedding. 
\fi

==> theory2.tex <==
\section{Understanding of VAE as Rate-distortion optimization of transform codig}

This section shows the relation between VAE and transform coding.  First, the mapping hypothesis between VAE  and the implict orthonormal transform is presented.  Then we describe both theoretical analysis and  expected observations.

\subsection{Hypothetical mapping of VAE to isometric space}
\label{SEC_HYPO}
In this section, the hypothetical mapping between VAE space and isometric space is presented. Figure \ref{fig:two} shows the hypothetical mapping.  For a given dataset space $S_{data}:\bm x \in  \mathbb{R}^m$ and metrics $D({\bm x}_a,{\bm x}_b)$, it is assumed that an implicit KLT (PCA)-like orthonormal transform exists as a result of Rate-distortion optimization.  Because of orthonormality, the implicit transformed space $S_{Iso}:\bm y \in  \mathbb{R}^m$ is isometric, and  $D({\bm x}_a,{\bm x}_b) = {\| {\bm y}_a - {\bm y}_b \|_2}^2$ holds where ${\bm x}_a,{\bm x}_b$ are sampled data and ${\bm y}_a,{\bm y}_b$ are their mapping to $S_{Iso}$. The value of probability measured in both $S_{data}$ and $S_{Iso}$ spaces are also the same because of constant Jacobian determinant between two spaces. The variance of each transformed variable $y_j (j=[1..m])$ will show the impact on the data space like PCA. 
%
Then the implicit isometric space $S_{Iso}$ is nonlinearly scaled to the VAE anisometric orthogonal space  $S_{VAE}: \bm z \in  \mathbb{R}^n$ on a variable-by-variable basis. Let $P(y_j)$ and $P(z_j)$ be probabiliy distribution of i-th varible in both $S_{Iso}$ and $S_{VAE}$.
Each variable $y_j$ is non-linearly scaled to $z_j$ such that $\mathrm{d}{z_j}/\mathrm{d}{y_j}= P(y_j)/P(z_j)$ to fit the cumulative distribution. In PCA, variables with small variance can be omitted for analysis. In image compression, coeffients for higher coefficients can be also discarded without significant degradation. From these analogies,  variables in $S_{Iso}$ with small variances are discarded.

\begin{figure}[h]
  \begin{center}
   \includegraphics[width=80mm]{figs/model.jpg}
%   \includegraphics{RDO.jpg}
  \end{center}
  \caption{Mapping of VAE to implicit orthonorml transform.}
  \label{fig:two}
\end{figure}

%\subsection{Theoretical analysis and expected observation}
%In this section, the theoretical analysis of the hypothesis is presented, then  expected observation is shown. In our analysis, ELBO of VAE in Eq.(\ref  {EQ_ELBO}) is interpreted to RDO cost of transfrom coding in Eq.(\ref  {EQ_RDO}). 
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Interpretation of ELBO to RDO cost}
\label{ELBOAnalysis}
%In this section, the theoretical analysis of the hypothesis is presented, then  expected observation is shown. In our analysis, ELBO of VAE in Eq.(\ref  {EQ_ELBO}) is interpreted to RDO cost of transfrom coding in Eq.(\ref  {EQ_RDO}). 
In this section, we reformulate the notation of ELBO for later theoretical analys.
%
First, the reformulation of reconstructon loss is explained. 
%
%Let decoded data $\hat {\bm x}$ and its i-th dimention value $\hat {x_i}$ in section \ref{sec:VAE} be replaced by $\bm x + \delta \bm x$ and $x_i + \delta \hat {x_i}$ respectively. 
$D(\bm x_a, \bm x_b)$ denotes a loss metrics between $\bm x_a$ and $\bm x_b$.
%
Let $ \breve {\bm x}$ be $Dec_{\theta}(\bm \mu)$.
%
%\citet{VAEPCA} shows that $D(\bm x, \hat {\bm x}) = D(\bm x, \breve {\bm x}) + D(\breve {\bm x}, \hat {\bm x})$ holds. Here, the first term encourages $Dec_{\theta}({\bm \mu}_{\bm x}) \sim \bm x$, and we assume this is optimized in the later analysis. The second term controls ${\bm \sigma}_{\bm x}$, and is expanded as follows.
\citet{VAEPCA} shows that $D(\bm x, \hat {\bm x}) = D(\bm x, \breve {\bm x}) + D(\breve {\bm x}, \hat {\bm x})$ holds. Here, the first term encourages $|Dec_{\theta}({\bm \mu}_{\bm x}) - \bm x|^2 \rightarrow 0$, and we assume this is zero for easy analysis here. Because the first term is only responsible for the reconstruction, the cost function of the first term can be different from the second term.

The second term $D(\breve {\bm x}, \hat {\bm x})$, which controls ${\bm \sigma}_{\bm x}$, is expanded as follows.
%
$\delta \bm x$ denotes $\hat {\bm x} - \breve {\bm x} $.
%
Generally, $D(\breve {\bm x}, \hat {\bm x})$ can be approximated by ${}^t{\delta \bm x} \ {\bm G}_{\bm x}  {\delta \bm x} + C_{\bm x}$ where ${\bm G}_{\bm x}$ and $C_{\bm x}$ are a $\bm x$ dependent positive definite metric tensor and a constant respectively. 
%Then Generally, the reconstruction loss can be approximated by ${}^t{\delta \bm x} \ {\bm G}_{\bm x}  {\delta \bm x} + C_{\bm x}$ form where ${\bm G}_{\bm x}$ and $C_{\bm x}$ are a $\bm x$ dependent positive definite metric tensor and a constant respectively, and 
%
For instance, Eq.(\ref{EQ_Bernoulli}) can be approximated as follows by using $\log (1+x) = x - x^2/2 + O(x^3)$ expansion.
% 
\begin{eqnarray}
\label{EQ_ApxBernoulli}
Eq.(\ref{EQ_Bernoulli}) 
\sim \sum_{i=1}^{m} - \left( {x_i}^{-1}+ \left( 1 - x_i \right)^{-1} \right) {\delta {x_i}}^2 / 2 \nonumber \\
+  \sum_{i=1}^{m} \left( x_i \log{{x_i}} + (1 - x_i) \log {(1 - {x_i})}\right)  %\nonumber \\
%+  \sum_{i=1}^{m} \left( x_i \log{{x_i}} + (1 - x_i) \log {(1 - {x_i})} +O \left ( \left (\frac {\delta x_i}{ x_i} \right)^3 \right)\right)  %\nonumber \\
%+ \sum_{i=1}^{m} \left( O \left ( \left (\frac {\delta x_i}{ x_i} \right)^3 \right) + O \left ( \left ( \frac {\delta  x_i}{1 - x_i} \right)^3 \right) \right)
%+  \sum_{i=1}^{m} \left( x_i \log{{x_i}} + (1 - x_i) \log {(1 - {x_i})} \right)  + \nonumber \\
%+ \sum_{i=1}^{m} \left( O \left ( \left (\frac {\delta x_i}{ x_i} \right)^3 \right) + O \left ( \left ( \frac {\delta  x_i}{1 - x_i} \right)^3 \right) \right)
\end{eqnarray}
%
Accordingly, $C_{\bm x}$ is the second term, and ${\bm G}_{\bm x}$ is denoted by
%
\begin{eqnarray}
\bm G_{\bm x} = 
  \left(
    \begin{array}{ccc}
      \frac{1}{2}\left(\frac{1}{x_1}+\frac{1}{1-x_1}\right) & 0 & \ldots \\
      0 & \frac{1}{2}\left(\frac{1}{x_2}+\frac{1}{1-x_2}\right) & \ldots \\
      \vdots & \vdots & \ddots  \\
    \end{array}
  \right) 
\end{eqnarray}
%
In case of Eq.(\ref{EQ_Gaus}), It is obvious that $\bm G_{\bm x} =  (1 / 2 {\sigma}^2) \ \bm I$ where $\bm I$ denotes an identity matrix, and $C_{\bm x}$ is the second term of the last equation in Eq.(\ref{EQ_Gaus}).
%
Then the average of reconstruction loss is calculated. Let ${\bm x}_{z_j}$ be $\mathrm{d}{\bm x}/\mathrm{d}{z_j}$, and $\delta z_j \sim N(0,\sigma_{j({\bm x})})$ be a added noize in i-th dimmention of $\bm z$. As shown in \citet{VAEPCA}, ${\delta \bm x}$ is approximated by
%
\begin{eqnarray}
{\delta \bm x} \sim \sum_{j=1}^{n} \delta {z_j} \ {{\bm x}_{z_j}}
\end{eqnarray}
%
Because $ \delta {z_j}$ and $ \delta {z_k}$ for $j \neq k$ are independent, the average of reconstruction loss is reformulated by
%
\begin{eqnarray}
\label{EQ_LSAPX}
\underset{{\bm z} \sim q_{\phi}(\bm z | \bm x)}{E} \left[ {}^t{\delta \bm x} \ {\bm G}_{\bm x} {\delta \bm x} \right] 
%\underset{\underset{q_{\phi}(\bm z | \bm x)}{\bm z \sim}}{E} \left[ |D_\theta(\bm z)- D_\theta(\bm \mu)|^2 \right] =
= \sum_{j=1}^{n}{{\sigma}_{j({\bm x})}}^2 \ {}^t{{\bm x}_{z_j}} \bm G_x {{\bm x}_{z_j}}
\end{eqnarray}

%Second, the KL-divergence is reformulated as the rate shown in Eq.\ref{EQ_PandR}. Let $P_{\mu \sigma}$ and $R_{\mu \sigma}$ be the probability and rate of a quantized symbol with mean $\mu$ and coding noise $\sigma ^ 2$ in  a latent variable $z \sim N(0,1)$. Let $T$ be a quntization step with coding noise $\sigma ^ 2$, and $T = 2 \sqrt{3} \sigma$ holds from Eq.\ref{EQ_Noise}. As shown in Fig.\ref{fig:ProbAcc}, $P_{\mu \sigma}$ is denoted by $\int _{\mu - T/2}^{\mu + T/2} p(z) \mathrm{d}z$ where $p(z)$ is $N(0,1)$. By using Simpson's numerical integration method and $e^x = 1+x+O(x^2)$ expantion, $P_{\mu \sigma}$ is approximated by 
%
Second, the KL-divergence is reformulated as the rate shown in Eq.\ref{EQ_PandR}. 
Let $P_{z_j}$ and $R_{z_j}$ be the probability and rate to encode $z_j \sim N(0,1)$ with mean $\mu_{j({\bm x})}$ and coding noise ${\sigma_{j({\bm x})}} ^ 2$ using uniform quantization. Let $T$ be a quntization step with coding noise ${\sigma_{j({\bm x})}} ^ 2$, and $T = 2 \sqrt{3} {\sigma _{j({\bm x})}}$ holds from Eq.\ref{EQ_Noise}. As shown in Fig.\ref{fig:ProbAcc}, $P_{z_j}$ is denoted by $\int _{\mu_{j({\bm x})} - T/2}^{\mu_{j({\bm x})} + T/2} p(z_j) \mathrm{d}z_j$ where $p(z_j)$ is $N(0,1)$. By using Simpson's numerical integration method and $e^x = 1+x+O(x^2)$ expantion, $P_{z_j}$ is approximated by 
%
\begin{eqnarray}
\label{EQ_Pms}
P_{z_j} 
\sim  \frac{T}{6} \left(p ({\mu_{j({\bm x})}} - {\textstyle \frac{T}{2}} ) + 4p ({\mu_{j({\bm x})}} )+p ({\mu_{j({\bm x})}} +  {\textstyle \frac{T}{2}} ) \right) \nonumber \\
%&=&  \frac{T}{6 \sqrt{2 \pi}} \left(e ^{-\frac{\left({\mu} - T/2 \right)^2}{2}} + 4 e^{- \frac{ {\mu}^2}{2}}  +e ^{-\frac{\left({\mu} + T/2 \right)^2}{2}} \right) \nonumber \\
=  \frac{T p \left({\mu_{j({\bm x})}}  \right)}{6} \biggl(4 + e ^\frac{ 4 \mu_{j({\bm x})} T  - T^2}{8}  +  e ^\frac{ -4 \mu_{j({\bm x})} T  - T^2}{8} \biggr ) \hspace{3mm} \nonumber \\
\sim T p \left({\mu_{j({\bm x})}}  \right) \left( 1 - \frac{T^2}{24} \right) \hspace{35mm} \nonumber \\ 
= \sqrt{\frac{6}{\pi}} {\sigma_{j({\bm x})}} \ e^{ - ({\mu_{j({\bm x})}}^2)/{2}} \left( 1 - \frac{{\sigma_{j({\bm x})}}^2}{2} \right)  \hspace{15mm}
\end{eqnarray}
\begin{equation}
\ %Dummy
\end{equation}
%
\if0
\begin{eqnarray}
\label{EQ_Pms}
P_{\mu\sigma} 
&\sim&  \frac{T}{6} \left(p \left({\mu} - T/2 \right) + 4p \left({\mu}  \right)+p \left({\mu} + T/2 \right) \right) \nonumber \\
%&=&  \frac{T}{6 \sqrt{2 \pi}} \left(e ^{-\frac{\left({\mu} - T/2 \right)^2}{2}} + 4 e^{- \frac{ {\mu}^2}{2}}  +e ^{-\frac{\left({\mu} + T/2 \right)^2}{2}} \right) \nonumber \\
&=&  \frac{T e^{ - \frac{{\mu}^2}{2}}}{6 \sqrt{2 \pi}} \left(4 + e ^{ \mu T /2 - T^2/8}  +  e ^{- \mu T /2 - T^2/8} \right ) \nonumber \\
&\sim& \frac{T e^{ - \frac{{\mu}^2}{2}}}{\sqrt{2 \pi}} \left( 1 - \frac{T^2}{24} \right) \nonumber \\ 
&=& \sqrt{\frac{6}{\pi}} \sigma e^{ - \frac{{\mu}^2}{2}} \left( 1 - \frac{\sigma^2}{2} \right)
\end{eqnarray}
\fi
By using $\log (1+x) = x + O(x^2)$, $R_{\mu\sigma}$ is derived by 
%
\begin{eqnarray}
\label{EQ_Rms}
R_{z_j} 
= -\log P_{z_j} \hspace{44mm} \nonumber \\
\sim -\frac{1}{2}\left( {\mu _{j({\bm x})}}^2 + {\sigma_{j({\bm x})}} ^2 - \log {\sigma_{j({\bm x})}}^2 - \log \frac{6}{\pi} \right)
\end{eqnarray}
%
\if0
\begin{eqnarray}
\label{EQ_Rms}
R_{z_j} 
&=& -\log P_{z_j} \nonumber \\
&\sim& -\frac{1}{2}\left( {\mu _{j({\bm x})}}^2 + {\sigma_{j({\bm x})}} ^2 - \log {\sigma_{j({\bm x})}}^2 - \log \frac{6}{\pi} \right)
\end{eqnarray}
\fi
%
When Eq.\ref{EQ_DKL} and Eq.\ref{EQ_Rms} are compared, both equations are equivalent except a small consant difference $(1-\log(6/\pi))/2 \sim 0.176$ for each dimension. 
As a result, KL-divergence for j-th dimention can be considered as the rate to encode $z_j$ with mean ${\mu _{j({\bm x})}}$ and noise ${\sigma_{j({\bm x})}} ^2$.
To make theoretical analysis easier, we use simpler form $P_{z_j} = T \ p(z_j) = 2 \sqrt{3} {\sigma_{j({\bm x})}} \  p(z_j)$ in Fig.\ref{fig:ProbAprx} instead of Eq.\ref{EQ_Pms} in the later analysis.
As a reslut, $D_{KL}(\cdot)$ is reformulated by
%
\if0
\begin{eqnarray}
D_{KL}(\cdot)&=&\sum_{j=1}^{n}-\log(2 \sqrt{3} \  \sigma_{j({\bm x})} \ p(z_j)) \nonumber \\
%&=& -\log \left ( \prod _{j=1}^{n} {\sigma}_{\bm xj} \  p(z_j)\right ) -n \log (2 \sqrt{3}) \nonumber \\
&=& -\sum_{j=1}^{m} \log \left ({\sigma}_{\bm xj} \  p(z_j) \right ) -n \log (2 \sqrt{3}) \nonumber \\
&=& -\log \bigl ( p(\bm z) \prod _{j=1}^{n} {\sigma}_{\bm xj} \bigr )-n \log (2 \sqrt{3})
\end{eqnarray}
\fi
%
% 
\begin{eqnarray}
\label{EQ_KLAPX}
-D_{KL}(\cdot)= \sum_{j=1}^{n}-\log(2 \sqrt{3} \ \sigma_{j({\bm x})} \ p(z_j))\hspace{19mm} \nonumber \\
%= -\log \left ( \prod _{j=1}^{n} {\sigma}_{j({\bm x})} \  p(z_j)\right ) -n \log (2 \sqrt{3}) \hspace{2mm} \nonumber \\
= -\sum_{j=1}^{m} \log \left ({\sigma}_{j({\bm x})} \  p(z_j) \right ) -n \log (2 \sqrt{3}) \hspace{5mm} \nonumber \\
= -\log \Bigl( p(\bm z) \prod _{j=1}^{n} {\sigma}_{j({\bm x})} \Bigr )-n \log (2 \sqrt{3}) \hspace{2mm} 
\end{eqnarray}
%
\begin{figure}[h]
% \begin{minipage}{0.5\hsize}
 \begin{minipage}[b]{.45\linewidth}
  \begin{center}
   \includegraphics[width=38mm]{figs/pms1.jpg}
  \end{center}
  \subcaption{Probability $P_{\mu \sigma}$}
  \label{fig:ProbAcc}
 \end{minipage}
　
% \begin{minipage}{0.5\hsize}
 \begin{minipage}[b]{.45\linewidth}
  \begin{center}
   \includegraphics[width=38mm]{figs/pms2.jpg}
  \end{center}
  \subcaption{Approximation of $P_{\mu \sigma}$}
  \label{fig:ProbAprx}
 \end{minipage}
%\caption{Probability $P_{\mu \sigma}$ for a symbol with mean $\mu$ and variance $\sigma^2$}
\caption{Probability for a symbol with mean $\mu$ and noise $\sigma^2$}
\label{fig:Probability}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Conditions to minimize ELBO}
\label{SEC_THEORY}
This section explains the minimun condition of ELBO. 
%First, the average of ELBO at $\bm x$ with regard to ${\bm z} \sim q_{\phi}(\bm z | \bm x)$ is formulated, and the condition of decoder's derivetive which minimize the average is clarilfied. 
%First, the condition of decoder's derivetive which minimize ELBO at $\bm x$ with regard to ${\bm z} \sim q_{\phi}(\bm z | \bm x)$ is clarified.
% Second, we show that optimal encoder which minimize ELBO with regard to ${\bm x} \sim p(\bm x)$ becomes the KLT(PCA)-like orhtonormal to the implicit latent space. 
%Let ${\bm x}_{z_j}$ be $\mathrm{d}{\bm x}/\mathrm{d}{z_j}$. By introducing $\bm G _x$ to the decoder's expansion shown in \citet{VAEPCA}, the average of reconstruction loss can be approximated by
%
%First, the condition of decoder's derivetive which minimize the averaged ELBO $L_{\bm x}$ at $\bm x$ with regard to ${\bm z} \sim q_{\phi}(\bm z | \bm x)$ is clarified.
First, the condition to minimize the averaged ELBO $L_{\bm x}$ at $\bm x$ w.r.t. ${\bm z} \sim q_{\phi}(\bm z | \bm x)$ is clarified.
%
%Let $L_{\bm x}$ be the averaged ELBO w.r.t. $q_{\phi}(\bm z | \bm x)$ at $\bm x$.
As a start point, the dimension of $\bm x$ and $\bm z$ are set to the same $(m=n)$.
By using Eqs.\ref{EQ_LSAPX} and \ref{EQ_KLAPX}, and neglecting constant offset, $L_{\bm x}$ is denoted by
%
\begin{eqnarray}
\label{EQ_RDOVAE}
L_{\bm x}=\underset{{\bm z} \sim q_{\phi}(\bm z | \bm x)}{E} \left [\log p_{\theta}(\bm x | \bm z) - \beta \ D_{KL}((q_{\phi}(\bm z | \bm x) \| p(z)) \right] \nonumber \\
=\sum_{j=1}^{m}{{\sigma}_{j({\bm x})}}^2 \ {}^t{{\bm x}_{z_j}} \bm G_x {{\bm x}_{z_j}} - {\beta} \log \Bigl ( p(\bm z) \prod _{j=1}^{m} {\sigma}_{j({\bm x})} \Bigr ) \hspace{5mm} \nonumber \\
=\sum_{j=1}^{m}{{\sigma}_{j({\bm x})}}^2 \ {}^t{{\bm x}_{z_j}} \bm G_x {{\bm x}_{z_j}} - {\beta} \log \Bigr ( p(\bm x) \left | \frac{\mathrm{d} \bm x}{\mathrm{d} \bm z} \right | \prod _{j=1}^{m} {\sigma}_{j({\bm x})} \Bigr )
\end{eqnarray}
%
\if0
\begin{eqnarray}
\label{EQ_RDOVAE}
%L=\sum_{j}^{n}{{\sigma}_{j}(\bm x)}^2 \frac{\partial{\bm x}}{\partial{z_j}}^T \bm G_x \frac{\partial{\bm x}}{\partial{z_j}} - \lambda \log p(\bm z) \prod _{j=1}^{n} {\sigma}_{j}(\bm x)\\
%L=\sum_{j}^{n}{{\sigma}_{(\bm x)j}}^2 \frac{\partial{\bm x}}{\partial{z_j}}^T \bm G_x \frac{\partial{\bm x}}{\partial{z_j}} - \lambda \log p(\bm z) \prod _{j=1}^{n} {\sigma}_{(\bm x)j}\\
%L=\sum_{j}^{n}{{\sigma}_{{\bm x},j}}^2 \frac{\partial{\bm x}}{\partial{z_j}}^T \bm G_x \frac{\partial{\bm x}}{\partial{z_j}} - \lambda \log \left ( p(\bm z) \prod _{j=1}^{n} {\sigma}_{\bm x,j} \right )\\
%=\sum_{j}^{n}{{\sigma}_{{\bm x},j}}^2 \frac{\partial{\bm x}}{\partial{z_j}}^T \bm G_x \frac{\partial{\bm x}}|{\partial{z_j}} - \lambda \log \left ( p(\bm z) | \frac{\mathrm{d} \bm x}{\mathrm{d} \bm z}\prod _{j=1}^{n} {\sigma}_{\bm x,j} \right )\\
%
L=\sum_{j=1}^{n}{{\sigma}_{j({\bm x})}}^2 \ \ {}^t{{\bm x}_{z_j}} \bm G_x {{\bm x}_{z_j}} - {\beta} \log \left ( p(\bm z) \prod _{j=1}^{n} {\sigma}_{j({\bm x})} \right )\nonumber \\
=\sum_{j=1}^{n}{{\sigma}_{j({\bm x})}}^2 \ \ {}^t{{\bm x}_{z_j}} \bm G_x {{\bm x}_{z_j}} - {\beta} \log \left ( p(\bm x) \left | \frac{\mathrm{d} \bm x}{\mathrm{d} \bm z} \right | \prod _{j=1}^{n} {\sigma}_{j({\bm x})} \right )
%L=\sum_{j}^{n}{{\sigma}_{j}(\bm x)}^2 \dot{{\bm x}_j}\\
%L=\sum_{j}^{n}{{\sigma}_{j}(\bm x)}^2 \partial{\bm x}/\partial{z_j}\\
%L=\sum_{j}^{n}{{\sigma}_{j}(\bm x)}^2 \frac{\partial{\bm x}}{\partial{z_j}}\\
%L=\sum_{j}^{n}{{\sigma}_{j}(\bm x)}^2 {\bm x}_{z_j}\\
\end{eqnarray}
\fi
%
Let $\Delta_{ij}$ be a cofactor of Jacobi matrix ${\mathrm{d} \bm x}/{\mathrm{d} \bm z}$ with regard to $ {\partial x_i}/{\partial z_j}$, and ${\tilde {\bm x}_{z_j}}$ be ${}^t (\Delta_{i1},\Delta_{i2}\cdots,\Delta_{in})$.
%
It is noted that ${}^t{{\bm x}_{z_j}} \cdot {\tilde {\bm x}_{z_j}}= \left | {\mathrm{d} \bm x}/{\mathrm{d} \bm z} \right | $ holds by definition, and ${}^t{{\bm x}_{z_j}} \cdot {\tilde {\bm x}_{z_k}}= 0$ holds for $j \neq k$ because it is derived by the determinant of singular matrix $(\cdots,{{\bm x}_{z_j}},\cdots,{{\bm x}_{z_j}},\cdots)$. Here,$\  \cdot $ denotes inner product.  
%
The derivative of $L_{\bm x}$ to derive the minimum is described by
%
%Let $\Delta_{ij}$ be a cofactor of Jacobi matrix $\frac{\mathrm{d} \bm x}{\mathrm{d} \bm z}$ with regard to $\frac {\partial x_i}{\partial z_j}$, and ${\tilde {\bm x}_{z_j}}$ be ${}^t (\Delta_{i1},\Delta_{i2}\cdots,\Delta_{in})$.
%
\begin{eqnarray}
\label{EQ_LPart}
\frac{\mathrm{d} L_{\bm x} \ }{\mathrm{d} {\bm x}_{z_j}} = 
2{{\sigma}_{j({\bm x})}}^2  \bm G_x {{\bm x}_{z_j}} - {\beta} {\left | \frac{\mathrm{d} \bm x}{\mathrm{d} \bm z} \right |}^{-1}{\tilde {\bm x}_{z_j}}
\end{eqnarray}
%
By setting Eq.\ref{EQ_LPart}  zero, multiplying ${}^t{{\bm x}_{z_j}}$ from the left, using Kronecker delta $\delta_{jk}$, and rearranging the equation, the condition to minimize $L_{\bm x}$ is clarified as the following orthogonal form of $\bm x_{z_j}$.
%
\begin{eqnarray}
\label{EQ_Ortho1}
\frac{2{{\sigma}_{j({\bm x})}}^2}{{\beta}} {}^t{{\bm x}_{z_j}} \bm G_x {{\bm x}_{z_k}} = \delta_{jk}
\end{eqnarray}
%
Next, implicit latent variable $\bm y$ and its i-th dimension $y_j$ are introduced by defining the derivetive between $y_j$ and $z_j$ as follows.
%
\begin{equation}
\label{EQ_Yscale}
\frac{\mathrm{d} y_j}{\mathrm{d} z_j} = \sqrt{\frac {\beta}{2}}{{\sigma}_{j({\bm x})}}^{-1}
%\mathrm{d} y_j / \mathrm{d} z_j = \sqrt{\frac {\beta}{2}}{{\sigma}_{j({\bm x})}}^{-1}
\end{equation}
%
${{\bm x}_{y_j}}$ denotes $\mathrm{d}{\bm x}/\mathrm{d} {y_j}$. 
%By applying  ${{\bm x}_{z_j}}= \mathrm{d} y_j / \mathrm{d} z_j \ {{\bm x}_{y_j}}$ to Eq.\ref{EQ_Ortho1}, the following orthonormal form in Hermitian inner product space with $\bm G _x$ is derived. 
By applying  ${{\bm x}_{z_j}}= \mathrm{d} y_j / \mathrm{d} z_j \ {{\bm x}_{y_j}}$ to Eq.\ref{EQ_Ortho1}, it is shown that ${{\bm x}_{y_j}}$ becomes orthonormal in the inner product space with a metric tensor $\bm G _{\bm x}$. 
%
\begin{eqnarray}
\label{EQ_Ortho2}
{}^t{{\bm x}_{y_j}} \bm G_{\bm x} {{\bm x}_{y_k}} = \delta_{jk}
\end{eqnarray}
%
At last,the condition to minimize the ELBO averaged w.r.t. $\bm x \sim p(\bm x)$ is examined.
% Because Jacobi matrix ${\mathrm{d}{\bm y}}/{ \mathrm{d} {\bm z}}$ is diagonal, the Jacobi determinant $|{\mathrm{d}{\bm y}}/{ \mathrm{d} {\bm z}}|$ is denoted by $\left ({\beta}/2 \right )^{n/2} \prod_{j=1}^n {{\sigma}_{j({\bm x})}}^{-1}$. 
%By applying Eq.\ref {EQ_Ortho1} and $p(z_j) = |{\mathrm{d}{y_j}}/{ \mathrm{d} {z_j}}|\  p(y_j)$ to Eq.\ref{EQ_RDOVAE}, the next cost function for ${\bm y}$  distribution is derived under the condition of Eq.\ref{EQ_Ortho2}.
Let $L \min _{\bm x}$ be the minimum value of $L_{\bm x}$ at $\bm x$. 
%
By applying Eq.\ref {EQ_Ortho1} to Eq.\ref{EQ_RDOVAE}, using the relation shown in Eq.\ref{EQ_RDOVAE}, aplying $p(z_j) = |{\mathrm{d}{y_j}}/{ \mathrm{d} {z_j}}|\  p(y_j)$, and using Eq.\ref{EQ_Yscale}, $L \min _{\bm x}$  is expanded as follows.
%
\begin{eqnarray}
\label{EQ_COSTX}
{L \min}_{\bm x}= \frac{n {\beta}}{2}  - {\beta} \sum_{j=1}^{m} \log \left ({\sigma}_{j({\bm x})} \  p(z_j) \right ) \hspace{15mm} \nonumber \\
= \frac{n {\beta}(1- \log ({\beta}/2))}{2}  -  {\beta} \sum_{j=1}^{m} \log p(y_j)
\end{eqnarray}
%
In the last equation of Eq.\ref{EQ_COSTX}, the first term is constat. As a result, the ELBO cost averaged w.r.t. $\bm x \sim p(\bm x)$ can be rewritten by
\begin{equation}
\label{EQ_COSTY}
%\underset{{\bm x} \sim p(\bm x)}{E} \left[-\sum_{j=1}^{n} \log p(y_j) \right]
\underset{{\bm x} \sim p(\bm x)}{E} \biggl[-\sum_{j=1}^{n} \log p(y_j) \biggr]
= -\sum_{j=1}^{n}\int p(y_j) \log p(y_j) \mathrm{d}y_j
\end{equation}
Here, the right term is the entropy of $\bm y$.  The orthonormal transform that minimizes entropy has been proven to be the Karhunen-Lo\`eve transform (KLT) \cite{KLTBook}.  After the KLT, the variance of each variable $y_j$ is the same as the eigenvalue of PCA.  Thus, latent variables with large variance are fufficient for the representation, and variables with smaller variances can be discarded without significant effect.  As a result, the hypothesis in the section \ref{SEC_HYPO} is proved.  It should be noted that KLT holds in the inner product space  with a metric tensor $\bm G_{\bm_x}$ as shown in Eq.\ref{EQ_Ortho2}.  Thus the  distribution of $\bm y$ is also affected by $\bm G_{\bm_x}$.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Expected observations from the theory}
\label{ExpObsv}
This section explaines the exptected observations in VAE which support the theory described in the section \ref{SEC_THEORY}.

The first exptected observation is the constant responsce of the latent variable to the data space. From Eq.\ref{EQ_Ortho1}, the following equation holds at any $\bm x$ and any dimention $j$ among the latent variables.  
$\bm u _j$ denotes a vector $(0,\cdots,\overset{\mathrm {}_{j-th}}{1},\cdots,0)$ where the j-th dimension is $1$, and other dimensions are $0$.  
$\epsilon$ denotes a minute displacement for the numerical differential. 
By using these notations, $D(Dec_\theta (\bm z), Dec_\theta (\bm z + \epsilon {\bm u}_j))/{\epsilon}^2$ is also denoted by $D^{\prime}_j(\bm z)$. Then the following equation holds.
%
\begin{eqnarray}
\label{EQ_OBSV1}
%{{\sigma}_{j({\bm x})}}^2 \frac{D(\tilde {\bm x}, Dec_\theta (\mu _{j({\bm x})} + \epsilon {\bm u}_j))}{{\epsilon}^2} \sim {{\sigma}_{j({\bm x})}}^2 \ {}^t{{\bm x}_{z_j}} \bm G_x {{\bm x}_{z_j}} \nonumber \\
%{{\sigma}_{j({\bm x})}}^2 D^{\prime}_j(\bm z) \sim {{\sigma}_{j({\bm x})}}^2 \ {}^t{{\bm x}_{z_j}} \bm G_x {{\bm x}_{z_j}} \nonumber \\
%= \frac{\beta}{2} \ \ {}^t{{\bm x}_{y_j}} \bm G_x {{\bm x}_{y_j}} = \frac{\beta}{2}  \hspace{2mm} (\mathrm{constant}) \hspace{3mm}
{{\sigma}_{j({\bm x})}}^2 D^{\prime}_j(\bm z) \sim 
 \frac{\beta}{2} \ \ {}^t{{\bm x}_{y_j}} \bm G_x {{\bm x}_{y_j}} = \frac{\beta}{2}  \hspace{2mm} (\mathrm{constant}) \hspace{3mm}
\end{eqnarray}
%
Here, the first term in Eq.\ref{EQ_OBSV1} can be evaluated numerically. If the values for different data $\bm x$ and dimension $j$ are observed as a constant, the existence of an implicit isometric space is supported.
%%%%

The second exptected observation is PCA-like feature.  The variance of i-th dimention implicit latent variable $y_j$ can be estimated by
\begin{eqnarray}
\label{EQ_OBSV2}
\int {y_j}^2 p(y_j) \mathrm{d} y_j &=&  \int \left ( \frac{\mathrm{d} y_j}{\mathrm{d} z_j}{z_j} \right) ^2 p(z_j) \mathrm{d} z_j  \nonumber \\
&=& \frac{\beta}{2} \int \left (\frac{z_j}{{\sigma}_{j({\bm x})}} \right) ^2 p(z_j) \mathrm{d} z_j   \nonumber \\
%&\sim&  \int {{\sigma}_{j({\bm x})}}^{-2} p(z_j) \mathrm{d} z_j \int  {z_j} ^2 p(z_j) \mathrm{d} z_j \nonumber \\
&\sim& \frac{\beta}{2} \int {{\sigma}_{j({\bm x})}}^{-2} p(z_j) \mathrm{d} z_j \underset{=1}{\underline {\int  {z_j} ^2 p(z_j) \mathrm{d} z_j}} \nonumber \\
&\sim& \frac{\beta}{2} \ \ \underset{\bm x \sim p(\bm x)}{E}[{{\sigma}_{j({\bm x})}}^{-2}]
\end{eqnarray}
%
$E[\ \cdot\ ]$ in the last equation, denoted by $\overline{{{\sigma}_{j({\bm x})}}^{-2}}$, can be derived from the data.  
If $\overline{{{\sigma}_{j({\bm x})}}^{-2}}$ show the importance of each latent variable like eigenvalue of PCA, the existence of implicit KLT(PCA)-like transform is supported. 
It is noted that the lowerbound of ELBO is given by $\sigma_{j({\bm x})} = 1$ and $ \mu _{j({\bm x})} = 0$. Thus, $\overline{{{\sigma}_{j({\bm x})}}^{-2}}$ with insignificant variables are also lower-bounded by $1$ under this condition.
%%%%

The third expected observation is the estimation of data probability. From Eq.\ref{EQ_Ortho2}, the Jacobian detarminant between $\bm y$ and $\bm x$ is derived by 
\begin{eqnarray}
\left | \frac{\mathrm{d} \bm y}{\mathrm{d} \bm x} \right| = |\bm G _ x| ^{1/2}
\end{eqnarray}
Jacobian matrix between $\bm z$ and $\bm y$ is diagonal, and its Jacobian determinant is given by the products of Eq.\ref{EQ_Yscale}. Here variables $y_j$ for $j > n$ are assumed to be insignificant, thus $\sigma_{j({\bm x})} = 1$ and $ \mu _{j({\bm x})} = 0$ hold. By applying these conditions, the probability of data $\bm x$ can be estimated by
%acobian determinants of $\mathrm{d} \bm x/\mathrm{d} \bm y$ and $\mathrm{d} \bm y/\mathrm{d} \bm x$If PCA feature holds, the variance of 
%
\begin{eqnarray}
\label{EQ_OBSV3}
%p(\bm x) = \left | \frac{\mathrm{d} \bm y}{\mathrm{d} \bm x} \right| \ p(\bm y) = \left | \frac{\mathrm{d} \bm y}{\mathrm{d} \bm x} \right| \left( \prod_{j=1}^{m} \frac{\mathrm{d} z_j}{\mathrm{d} y_j}\right) p(\bm z)   \hspace{8mm} \nonumber \\
p(\bm x) = \left | \frac{\mathrm{d} \bm y}{\mathrm{d} \bm x} \right| \prod_{j=1}^{m} p(y_j) = \left | \frac{\mathrm{d} \bm y}{\mathrm{d} \bm x} \right| \prod_{j=1}^{m} \left(  \frac{\mathrm{d} z_j}{\mathrm{d} y_j} p(z_j)\right)   \nonumber \\
= (2/\beta)^{\frac{m}{2}} (2 \pi)^{\frac{n-m}{2}}|\bm G _ x| ^{1/2} \prod_{j=1}^{n} \left( {{\sigma}_{j({\bm x})}}  p(\bm z_j)\right) \nonumber \\
\propto |\bm G _ x| ^{1/2}  \prod_{j=1}^{n} \left({{\sigma}_{j({\bm x})}}  p(\bm z_j)\right) \hspace{25mm}
\end{eqnarray}
If $p(\bm x)$ is proportional to the last equation, it is supposed that the scaling between $z_j$ and $y_j$ is given by Eq.\ref{EQ_Yscale}.

